Paraphrasing Is All You Need for Novel Object Captioning

Novel object captioning (NOC) aims to describe images containing objects without observing their ground truth captions during training. Due to the absence of caption annotation, captioning models cannot be directly optimized via sequence-to-sequence training or CIDEr optimization. As a result, we present Paraphrasing-to-Captioning (P2C), a two-stage learning framework for NOC, which would heuristically optimize the output captions via paraphrasing. With P2C, the captioning model first learns paraphrasing from a language model pre-trained on text-only corpus, allowing expansion of the word bank for improving linguistic fluency. To further enforce the output caption sufficiently describing the visual content of the input image, we perform self-paraphrasing for the captioning model with fidelity and adequacy objectives introduced. Since no ground truth captions are available for novel object images during training, our P2C leverages cross-modality (image-text) association modules to ensure the above caption characteristics can be properly preserved. In the experiments, we not only show that our P2C achieves state-of-the-art performances on nocaps and COCO Caption datasets, we also verify the effectiveness and flexibility of our learning framework by replacing language and cross-modality association models for NOC. Implementation details and code are available in the supplementary materials.

==> sections/2_connection.tex <==
\section{Connecting fluency, fidelity and adequacy with perplexity and mutual information}
\label{sec:connection}

We first discuss how fluency, fidelity, and adequacy can be fundamentally and technically related to perplexity and mutual information \frank{in or of what?}. For caption fluency, one would expect that the image caption to be linguistically natural and fluent. That is, the NOC model not only requires to capture the occurrence of novel-object vocabularies, the associated collocations such as verbs or modifiers are expected to be properly utilized. Thus, given the context containing novel-object vocabularies as $\tilde{\mathrm{y}}$ and the associated collocations as $\hat{\mathrm{y}}$, we define fluency as the probability of the NOC model which correctly predicts the collocation given the novel image context $\prod_{i=1}^N p(\hat{\mathrm{y_i}}|\tilde{\mathrm{y}})$ ($N$ as the number of collocations) \frank{I didn't see any definition of perplexity?}. In natural language processing, masked language models are widely applied to predict $N$ masked word $\hat{\mathrm{y}}$ given the context $\tilde{\mathrm{y}}$, whose perplexity can be defined as inverse probability of the prediction, i.e.,
\begin{equation}
    \label{perplexity}
    \begin{aligned}
        \sqrt[N]{\frac{1}{p(\hat{\mathrm{y}}_1, \hat{\mathrm{y}}_2, ... \hat{\mathrm{y}}_N|\tilde{\mathrm{y}})}} = (\prod_{i=1}^N p(\hat{\mathrm{y_i}}|\tilde{\mathrm{y}}))^{-\frac{1}{N}}.
    \end{aligned}
\end{equation}
Thus, to achieve high linguistic fluency, the language model is expected to produce captions with low perplexity.

We now relate fidelity and adequacy in image captions to \frank{mutual information}. We start by defining the probability of an object appearing in the images as $p(x)$, and the probability of an object mentioned by the captions as $p(y)$ \frank{(What's the relation between x and y?)}. Relevant objects $p(x,y)$ are defined as objects that are both included in the image and described by the associated caption. Since fidelity assesses whether the visual content presented in the produced caption is correct, it can be defined as the fraction of relevant objects among objects in captions $\frac{p(x,y)}{p(y)} = p(x|y)$. On the other hand, adequacy evaluates whether sufficient visual details have been expressed by captions, and it can be defined as the fraction of relevant objects among objects in an image $\frac{p(x,y)}{p(x)} = p(y|x)$. Thus, we can calculate the point-wise mutual information $pmi$ of an image $x$ and its caption $y$ as follows:
\begin{equation}
    \label{perplexity}
    \begin{aligned}
        pmi(x,y) \equiv log\frac{p(x,y)}{p(x)p(y)} = log\frac{p(x|y)}{p(x)} = log\frac{p(y|x)}{p(y)},
    \end{aligned}
\end{equation}
with mutual information as the expected value of point-wise mutual information. For the task of NOC, both $p(x)$ and $p(y)$ are fixed (i.e., determined by the dataset). Therefore, the above derivation implies that when the mutual information between an image and its captions increases, the resulting fidelity and adequacy would be jointly improved. 


==> sections/statement.tex <==
\section*{Ethics Statement}

We acknowledge that all authors of this work have read and commit to adhering to the ICLR code of ethics. Our work has no ethical concern.

\section*{Reproducibility Statement}

For reproducing our results in the experiment section, codes and training/testing scripts are provided in the supplementary materials.
